The Mechanical Neural Network(MNN) -- A physical implementation of a multilayer perceptron for education and hands-on experimentation

In this paper the Mechanical Neural Network(MNN) is introduced, a physical implementation of a multilayer perceptron(MLP) with ReLU activation functions, two input neurons, four hidden neurons and two output neurons. This physical model of a MLP is used in education to give a hands on experience and allow students to experience the effect of changing the parameters of the network on the output. Neurons are small wooden levers which are connected by threads. Students can adapt the weights between the neurons by moving the clamps connecting a neuron via a thread to the next. The MNN can model real valued functions and logical operators including XOR.

==> acronyms.tex <==
%
%
%
%
\newacronym{aaap}{aaap}{as affine as possible}

\newacronym{acm}{ACM}{Association for Computing Machinery}

\newacronym{acr}{ACR}{active camera relocalization}

\newacronym{ar}{AR}{Augmented reality}

\newacronym{dem}{DEM}{Digital Elevation Model}

\newacronym{dof}{DOF}{depth of field}

\newacronym{dorelu}{doReLU}{Double Rectified Linear Unit}

\newacronym{dslr}{DSLR camera}{digital single lens reflex camera}

\newacronym{eg}{EG}{Eurographics}

\newacronym{fsa}{FSA}{Farm Security Administration}

\newacronym{gcp}{GCP}{ground control point}

\newacronym{gif}{GIF}{Graphics Interchange Format}

\newacronym{gps}{GPS}{Global Positioning System}

\newacronym{hci}{HCI}{Human Computer Interaction}

\newacronym{hdri}{HDRI}{high-dynamic-range imaging}

\newacronym{hsi}{HSI}{habitat suitability model}

\newacronym{ieee}{IEEE}{Institute of Eletrical and Electronics Engineers}

\newacronym{insticc}{INSTICC}{Institute for Systems and Technologies of Information, Control and Communication}

\newacronym{js}{JS}{JavaScript}

\newacronym{lia}{LIA}{Little Ice Age}

\newacronym{mdia}{MDIA}{multi-data integrative analysis}

\newacronym{mlp}{MLP}{multilayer perceptron}

\newacronym{mnn}{MNN}{Mechanical Neural Network}

\newacronym{nasa}{NASA}{National Aeronautics and Space Administration}

\newacronym{ngs}{NGS}{U.S. National Geodetic Survey}

\newacronym{ppm}{PPM}{photopointmonitoring}

\newacronym{relu}{reLU}{Rectified Linear Unit}

\newacronym{siggraph}{SIGGRAPH}{Special Interest Group on Computer Graphics and Interactive Techniques}

\newacronym{sits}{SITS}{Satellite Image Time Series}

\newacronym{uav}{UAV}{unmanned aerial vehicle}

\newacronym{usgs}{USGS}{United States Geological Survey}

\newacronym{vr}{VR}{Virtual reality}

\newacronym{vrp}{VRP}{virtual repeat photography}

\newacronym{wave}{WAVE}{Wide-Area Visualisation environment}

\newacronym{wscg}{WSCG}{World Society for Computer Graphics}

\newacronym{wwi}{WWI}{World War I}

\newacronym{wwii}{WWI}{World War II}
